Reachability Analysis for FollowerStopper: Safety Analysis and Experimental Results

Motivated by earlier work and the developer of a new algorithm, the FollowerStopper, this article uses reachability analysis to verify the safety of the FollowerStopper algorithm, which is a controller designed for dampening stop- and-go traffic waves. With more than 1100 miles of driving data collected by our physical platform, we validate our analysis results by comparing it to human driving behaviors. The FollowerStopper controller has been demonstrated to dampen stop-and-go traffic waves at low speed, but previous analysis on its relative safety has been limited to upper and lower bounds of acceleration. To expand upon previous analysis, reachability analysis is used to investigate the safety at the speeds it was originally tested and also at higher speeds. Two formulations of safety analysis with different criteria are shown: distance-based and time headway-based. The FollowerStopper is considered safe with distance-based criterion. However, simulation results demonstrate that the FollowerStopper is not representative of human drivers - it follows too closely behind vehicles, specifically at a distance human would deem as unsafe. On the other hand, under the time headway-based safety analysis, the FollowerStopper is not considered safe anymore. A modified FollowerStopper is proposed to satisfy time-based safety criterion. Simulation results of the proposed FollowerStopper shows that its response represents human driver behavior better.

==> intro-old.tex <==
Recent research has shown that it is possible to dampen stop-and-go traffic waves on a ring road through the actions of one autonomous vehicle \cite{stern2018dissipation}\cite{wu2019flow}.  As a result, there has been a particular interest to investigate how to control the flow of traffic using a subset of vehicles that are under autonomous control. One such controller to do so, the FollowerStopper \cite{Rahul2018}, was applied at low speeds ($v\leq8 \text{m/s}$) as part of the Arizona Ring Experiment~\cite{wu2018arizona}, where it demonstrated effectiveness by significantly reducing emergent traffic waves through feedback control, based on the velocity (and relative distance) of the vehicle in front of the control vehicle \cite{stern2018dissipation}. The vehicle used for the control of the traffic stream, in this case, was a 2009 Ford Escape with additional sensing and actuation features installed~\cite{448}, which would not be possible to deploy at a reasonable cost and scale at a consumer level. 

Fortunately, several newer vehicles (e.g., since 2017) have standard features such as adaptive cruise control, lane-keeping assistance, and forward collision avoidance. These advancements provide two meaningful motivations for determining a wider deployment of velocity controllers that might have additional qualitative benefits that go beyond cruise control. First, would it be possible to safely field a controller like the FollowerStopper on existing vehicles, without the need to install additional sensors or computers in the vehicle? Second, could we use the data currently being obtained by on-vehicle sensors to configure and validate candidate controllers and analyze their safety?

Importantly, while the results of the Arizona Ring Experiment demonstrated the efficacy of the approach for traffic wave dampening, those results do not speak to the safety of the FollowerStopper controller in normal traffic scenarios. Specific questions on safety are (1) whether the FollowerStopper, as designed, is safe at the speeds for which it was originally tested, and (2) whether it would be safe at higher speeds. If it is not safe at higher speeds, what improvements can be made which would improve its safety envelope?

% This paper approaches these questions in the following ways: (1) How can we develop a safety analysis process that can guarantee whether or not the FS is safe and (2) given our analysis on the Follower-stopper, how can we improve the Follower-stopper in terms of safety such that it’s more robust in highway driving? 

\subsection*{Contribution of this work}
Our approach for (1) is the use of level-set methods to synthesize safe sets, and the use of driving data across hundreds of drives by human drivers to obtain the minimum and maximum accelerations for the growth of the level-sets. Throughout this work, we will \textit{continuously validate and improve the robustness of the safe sets} with real human driving data gathered over several months. These data will help us surmise whether our definition of safety and model choices for the analysis is valid. Our approach for (2) is to use results from (1) to propose a new design for the FollowerStopper for which observed driving data that come from known safe behaviors are used to determine the controller regions. We use these data to propose a change in the switching regions of the FollowerStopper that encourages a new safety metric of time-based headway, which was not a variable in previous deployments due to the low-speed threshold.
% the Follower-stopper to keep a more time-based headway in its driving.

% \subsection*{Contribution of this work}
% This paper uses reachability analysis to demonstrate that the existing design of the FollowerStopper controller is not safe at $v>8\;\mathrm{m/s}$, and that there exist scenarios even at low speeds where collisions may occur if aggressive braking of the lead vehicle was observed. 
% This paper demonstrates that while our model uses approximations of the vehicle's dynamics, that the boundaries of the safe sets are consistent with distance and velocity information gathered from human-driven vehicle data. Thus we conclude that the safety bounds of the controller are consistent with the safety bounds of drivers who controlled the vehicle during data gathering, and surmise that a vehicle following our ego car would not see decelerations or accelerations that exceed the magnitudes of those of a human-driven vehicle. 

\subsection*{Organization}
In section \ref{sec:background}, we provide brief reviews of relevant works. We formulate the safety analysis for FollowerStopper in section \ref{sec:problemFormulation}. The distance-based safety set of FollowerStopper is shown in section \ref{sec:safetyAnalysis4FollowerStopper}, along with comparing against driving data. Time headway based safety analysis, which factors in the absolute speed of the subject vehicle is shown in section \ref{sec:safetSetWithTimeHeadway}. To meet time headway based safety, FollowerStopper is modified and verified with time headway safety analysis in section \ref{sec:Modify_FollowerStopper}. Section \ref{sec:conclusions} concludes this article.
